OmniNOCS: A unified NOCS dataset and model for 3D lifting of 2D objects

We propose OmniNOCS, a large-scale monocular dataset with 3D Normalized Object Coordinate Space (NOCS) maps, object masks, and 3D bounding box annotations for indoor and outdoor scenes. OmniNOCS has 20 times more object classes and 200 times more instances than existing NOCS datasets (NOCS-Real275, Wild6D). We use OmniNOCS to train a novel, transformer-based monocular NOCS prediction model (NOCSformer) that can predict accurate NOCS, instance masks and poses from 2D object detections across diverse classes. It is the first NOCS model that can generalize to a broad range of classes when prompted with 2D boxes. We evaluate our model on the task of 3D oriented bounding box prediction, where it achieves comparable results to state-of-the-art 3D detection methods such as Cube R-CNN. Unlike other 3D detection methods, our model also provides detailed and accurate 3D object shape and segmentation. We propose a novel benchmark for the task of NOCS prediction based on OmniNOCS, which we hope will serve as a useful baseline for future work in this area. Our dataset and code will be at the project website: https://omninocs.github.io.

==> figures/ious_vs_inst.tex <==
\begin{figure}[t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  \includegraphics[width=0.9\linewidth]{images/size_err_vs_instances.png}
   \caption{\small{Comparing the relative size errors of CubeRCNN vs our model as a function of the number of instances for the corresponding class. Our model without any class-specific parameters has lower size errors for less frequent classes.}}
   \label{fig:iou-vs-instances}
\end{figure}

==> figures/qual_nocs_indoors.tex <==
\begin{figure}[t]
    \includegraphics[width=\linewidth]{images/qual_nocs_indoor.png}
    \captionof{figure}
    {
    \small{
    Qualitative results of \textbf{\nocsmethod{}} model across various indoor datasets and object classes. Left column shows the input images and query 2D bounding boxes. The right image shows the predicted per object NOCS, segmentation, and 3D oriented bounding box from our model corresponding to each input query overlaid on the input image.
    }
    }\label{fig:qual_nocs_indoors}
\end{figure}%

==> figures/qualitative_ours_direct.tex <==
\begin{figure}[t]
    \includegraphics[width=\linewidth]{images/qualitative_ours_direct.jpg}
    \captionof{figure}
    {
    \small{
    Example results of \textbf{\boxmethod} model across various datasets and object classes. The left column shows the input images and query 2D bounding boxes. The right image shows the predicted per object 3D oriented bounding box from our model corresponding to each input query overlaid on the input image.
    }
    }\label{fig:qualitative_ours_direct}
\end{figure}%

==> tables/ablation_nocs.tex <==
\begin{table}[h!]
\centering
\centering
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c c c}
 \hline
 Method & 2D Mask IoU & NOCS PSNR (dB) \\ [0.5ex]
 \hline
 \nocsmethod & \textbf{85.2} & \textbf{24.3}  \\ 
  w/o DPT & 83.1 & 22.8 \\
  w/o SS loss & -  & 24.1 \\
  w/o hourglass mask head & 83.7 & 24.2 \\ [1ex] 
\hline
\end{tabular}
}
\caption{\small{Impact on the quality of the instance mask and NOCS map produced by the model when dropping different components of our architecture or losses.}}

\label{table:ablation-nocs}
\end{table}

\begin{table}[h!]
\centering
\centering
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1}
\begin{tabular}{l|c c c}
 \hline
 Method & Depth error & Size Error & Orientation error \\ [0.5ex]
 \hline
 \boxmethod & \textbf{1.45} & \textbf{0.22} &  \textbf{0.64} \\ 
  w/o DPT & 1.76 & 0.23 & 0.69 \\
 \hline
\end{tabular}
\caption{\small{Impact on the quality of the 3D bounding boxes produced by {\boxmethod} when not using DPT. Note that the depth error here is measured in our virtual camera space and is not in meters, and the orientation error is a Chamfer loss (meters) between the the ground truth and predicted box corners that only differ in orientation.}} 

\label{table:ablation-box}
\end{table}

==> tables/baselines.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1}
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc|ccc|c}
\toprule
 & \multicolumn{4}{c}{Direct regress}
 & \multicolumn{3}{c}{Coord+PnP}
 & Ours
 \\
  \cmidrule(lr){2-5}
  \cmidrule(lr){6-8}
  \cmidrule(lr){9-9}
 &
  \rot{M3D-RPN~\cite{brazil2019m3d}} &
  \rot{FCOS3D~\cite{wang2021fcos3d}} &
  \rot{CubeRCNN~\cite{brazil2023omni3d}} &
  \rot{MonoDETR~\cite{zhang2022monodetr}} &
  \rot{NOCS~\cite{Wang_2019_CVPR}} &
  \rot{MonoRUn~\cite{monorun2021}} &
  \rot{EProPnP~\cite{chen2022epro}} &
  \rot{} \\
\cmidrule{2-9}
%                           M3   FC   CR   MD   NC   MR   EP   Ours
{1) Multi-dataset}        & \n & \n & \y & \n & \n & \n & \y & \y  \\
{2) No class-specific params}       & \n & \n & \n & \n & \n & \y & \y & \y  \\
{3) Full Orientation}     & \n & \n & \n & \n & \y & \n & \y & \y  \\
{4) Shape Reconstruction} & \n & \n & \n & \n & \y & \n & \n & \y  \\
%{5) Text Embedding}       & \n & \n & \n & \n & \n & \n & \n & \y  \\
\bottomrule
\end{tabular}
%}
\vspace{-.5em}
\caption{
    \textbf{Comparison of features with related methods.}
    The rows indicate whether each method:
    1) generalizes to different datasets and camera parameters,
    2) does not contain class-specific parameters,
    3) predicts a full canonical pose (3DoF orientation) for each class,
    4) reconstructs the object shape, e.g., including depth + segmentation
%    5) predicts texts embeddings for classes.
\vspace{-5mm}
}
\label{tab:baselines}
\end{table}

% Notes: 

% M3D-RPN. Results on KITTI only, orientation is a single angle

% FCOS3D. Results on nuScenes only, orientation is a single angle 
% method seems mainly class agnostic: "Detection heads are shared among multi-level feature maps except that three scale factors are used to differentiate some of their final regressed results, including offsets, depths, and sizes, respectively"

% MonoDETR. Results on KITTI only. orientation not super clear but I think it is a single angle
% class agnostic (Y): instead of using 2D detectors they "guide the whole detection process by contextual depth cues", predicting category in the detection head.
% shape: depth is predicted but not segmentation

% MonoRUN. Results on KITTI only. orientation single yaw angle. shape: no segmentation

% EProPNP. Results on KITTI and LineMOD. Orientation quaternion. Shape: no segmentation


% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3pt}
% \def\arraystretch{1}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc|cccc|ccc|cc|c}
% \toprule
%  & \multicolumn{5}{c}{Direct regression}
%  & \multicolumn{4}{c}{NOCS methods}
%  & \multicolumn{3}{c}{Latent}
%  & \multicolumn{2}{c}{NOCS+PnP}
%  & Ours
%  \\
%  \cmidrule(lr){2-6}
%  \cmidrule(lr){7-10}
%  \cmidrule(lr){11-13}
%  \cmidrule(lr){14-15}
%  \cmidrule(lr){16-16}
%  &
%   \rot{M3D-RPN~\cite{brazil2019m3d}} &
%   \rot{FCOS3D~\cite{wang2021fcos3d}} &
%   \rot{CubeRCNN~\cite{brazil2023omni3d}} &
%   \rot{MonoDETR~\cite{Lin21iccv_BARF}} &
%   \rot{~\cite{Jain21iccv_DietNeRF}} &
%   \rot{NOCS~\cite{Wang_2019_CVPR}} &
%   \rot{MonoRUn~\cite{monorun2021}} &
%   \rot{EProPnP~\cite{chen2022epro}} &
%   \rot{\cite{Chen21iccv_MVSNeRF}} &
%   \rot{CodeNeRF~\cite{Jang21iccv_CodeNeRF}} &
%   \rot{NeRF-VAE~\cite{Kosiorek21icml_NeRF_VAE}} &
%   \rot{LFN~\cite{sitzmann2021lfn}} &
%   \rot{NRW~\cite{nrw}} &
%   \rot{MonoRUn~\cite{monorun2021}} &
%   \rot{\lit{}} \\
% \cmidrule{2-16}
% {1) Multi-dataset}      & \n & \n & \y & \y & \y & \y & \y & \y & \y & \n & \n & \n & \y & \y & \y \\
% {2) Class-agnostic}     & \y & \y & \y & \y & \y & \y & \y & \y & \y & \y & \y & \y & \n & \n & \y \\
% {3) Template-free}     & \y & \y & \y & \y & \y & \y & \y & \y & \y & \y & \y & \y & \n & \n & \y \\
% {4) Canonical Pose}            & \n & \y & \n & \n & \n & \n & \n & \n & \n & \n & \n & \y & \n & \n & \y \\
% {5) Object reconstruction}      & \n & \n & \y & \n & \n & \n & \n & \n & \n & \n & \n & \n & \n & \n & \y \\
% {6) Text embedding}        & \n & \n & \n & \n & \n & \n & \n & \n & \n & \y & \y & \y & \n & \n & \y \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-.5em}
% \caption{
%     \textbf{Comparison of features with prior methods.}
%     The rows indicate whether each method:
%     1) generalizes to different datasets and camera parameters,
%     2) does not contain class-specific parameters,
%     3) predicts a canonical pose (orientation) for each class,
%     4) reconstructs the object shape,
%     5) predicts texts embeddings for classes.
% \vspace{-5mm}
% }
% \label{tab:baselines}
% \end{table}

% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c| } 
%  \hline
%  Method & Multi-dataset & Class-agnostic & Canonical & Reconstruct & Text \\ 
%  \hline
%  CubeRCNN & \cmark & \xmark & \xmark & \xmark & \xmark \\ 
%  \hline
%  MonoRUN & \xmark & \cmark & \cmark & \cmark & \xmark \\ 
%  \hline
%  EPro-PNP & \xmark & \cmark & \cmark & \cmark & \xmark \\ 
%  \hline
%  Ours & \cmark & \cmark & \cmark & \cmark & \cmark \\ 
%  \hline
% \end{tabular}
% \end{center}


==> tables/exp_nuscenes.tex <==
\begin{table}[h!]
\centering
\centering
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1}
%\resizebox{\linewidth}{!}{
\begin{tabular}{l|c c c} 
 \hline
\multirow{2}{*}{Method} & mATE & mAOE & mASE \\  
  & (m) & (rad) & (\%) \\ [0.5ex] 
 \hline
 FCOS3D \cite{wang2021fcos3d} & 0.777 & 0.400 & \textbf{0.231} \\
 PGD \cite{wang2022probabilistic} & 0.675 & 0.399 & 0.236 \\ 
 EProPNP \cite{chen2022epro} & 0.676 & 0.363 & 0.263 \\
 EProPNP + TTA \cite{chen2022epro} & \textbf{0.653} & \textbf{0.319} & 0.255 \\ [0.5ex]
 \hline
 CubeRCNN \cite{brazil2023omni3d} & \textbf{0.671} & 1.000 & 0.289 \\
 \boxmethod & 0.881 & 0.573 & 0.300 \\
% \nocsmethod (Zero Shot) & \color{red} 0.605 & \color{red} 0.243 & \color{red} 0.359 & \\
 \nocsmethod (self-supervised) & 0.893 & \textbf{0.443} & \textbf{0.264} \\
 \hline
\end{tabular}
%}
\caption{\small{Comparison of 3D localization accuracy on the nuScenes dataset. Top half: single-dataset methods, lower half: multi-dataset methods. Note amongst multi-dataset methods, \textbf{\nocsmethod} gives the best orientation and size errors.}
\label{table:nuscenes}}
\end{table}


\begin{table}[h!]
\centering
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c c c c} 
 \hline
 Method & mATE (m) & mAOE (rad) & mASE (\%) & mIoU (\%)\\ [0.5ex] 
 \hline
 CubeRCNN \cite{brazil2023omni3d} &  \textbf{0.650} &  1.305 & \textbf{0.283} & 0.349 \\
 % (these were not per class average)
 %\boxmethod & 0.9845 & 3.598 & 0.359 & \\ [1ex]
 \boxmethod & 0.790 & 0.573 & 0.301 & 0.280 \\
%\nocsmethod & \textbf{0.2987} & \textbf{2.114} &  & \\ [1ex]
\nocsmethod & 0.887 & \textbf{0.558} & 0.291 & \textbf{0.377} \\ [1ex]
 \hline
\end{tabular}
}
\caption{\small{Comparison of 3D localization accuracy on the KITTI validation set for all classes. mIoU and orientation error only uses the predicted yaw orientation component.}}
\label{table:kitti-localize}
\end{table}

